Vector OFDM Transmission over Non-Gaussian Power Line Communication Channels

Most of the recent power line communication (PLC) systems and standards, both narrow-band and broadband, are based on orthogonal frequency-division multiplexing (OFDM). This multiplexing scheme however suffers from the high peak-to-average power ratio (PAPR) which can considerably impact the energy efficiency, size and cost of PLC modems as well as cause electromagnetic compatibility (EMC) issues. This paper investigates the performance of vector OFDM (VOFDM), which has inherently better PAPR properties, over non-Gaussian broadband PLC channels equipped with two nonlinear preprocessors at the receiver. In addition, the low PAPR property of the VOFDM system is exploited to further enhance the efficiency of the nonlinear preprocessors. The achievable gains are studied in terms of the complementary cumulative distribution function of the PAPR, probability of noise detection error and the signal-to-noise ratio at the output of the nonlinear preprocessors. For comparison's sake, the performance of conventional OFDM systems is also presented throughout the paper. Results reveal that the proposed system is able to provide up to 2 dB saving in the transmit power relative to the conventional OFDM under same system conditions, which eventually also translates into a system that is more resilient to EMC limits, reduced cost and size of PLC modems. It is also shown that the achievable gains become more significant as the vector block (VB) size of the VOFDM system is increased.

==> sg_refs.ltx <==
% This file was created with JabRef 2.10.
% Encoding: Cp1252

@PREAMBLE{ "\newcommand{\noopsort}[1]{} " # "\newcommand{\printfirst}[2]{#1} " # "\newcommand{\singleletter}[1]{#1} " # "\newcommand{\switchargs}[2]{#2#1} " }


@Article{8Haffenden,
  Title                    = {Detection and removal of clipping in multicarrier receivers},
  Author                   = {O. P. Haffenden et al.},
  Journal                  = {Eur. patent appl. EP1043874},
  Year                     = {Oct. 2000, Bull. 20000/4}
}

@Article{Magazine11011,
  Title                    = {{IP}-centric high rate narrowband {PLC} for smart grid applications},
  Author                   = {Adebisi, B. and Treytl, A. and Haidine, A. and Portnoy, A. and Shan, R.U. and Lund, D. and Pille, H. and Honary, B.},
  Journal                  = {IEEE Commun. Mag.},
  Year                     = {2011},

  Month                    = {Dec. },
  Number                   = {12},
  Pages                    = {46 -54},
  Volume                   = {49}
}

@Article{Emad_Khaled13_1,
  Title                    = {Dynamic Peak-Based Threshold Estimation Method for Mitigating Impulsive Noise in Power-Line Communication Systems},
  Author                   = {Alsusa, E. and Rabie, K.M.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {Oct. 2013},
  Number                   = {4},
  Pages                    = {2201-2208},
  Volume                   = {28}
}

@Article{alsusa2013dynamic008,
  Title                    = {Dynamic peak-based threshold estimation method for mitigating impulsive noise in power-line communication systems},
  Author                   = {Alsusa, Emad and Rabie, Khaled M},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2013},

  Month                    = {Oct.},
  Number                   = {4},
  Pages                    = {2201--2208},
  Volume                   = {28}
}

@Article{PD_2,
  Title                    = {Multipath characterization of indoor power-line networks},
  Author                   = {D. Anastasiadou and T. Antonakopoulos},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2005},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = { 90-99},
  Volume                   = {20}
}

@Article{Andreadou10,
  Title                    = {Mitigation of Impulsive Noise Effect on the {PLC} Channel With {QC}-{LDPC} Codes as the Outer Coding Scheme},
  Author                   = {Andreadou, N. and Pavlidou, F-N},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2010},

  Month                    = {Jul.},
  Number                   = {3},
  Pages                    = {1440-1449},
  Volume                   = {25}
}

@Article{Andreadou09,
  Title                    = {{PLC} Channel: Impulsive Noise Modelling and Its Performance Evaluation Under Different Array Coding Schemes},
  Author                   = {Andreadou, N. and Pavlidou, F-N},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2009},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {585-595},
  Volume                   = {24}
}

@Article{SLM31,
  Title                    = {Reducing the Peak-to-Average Power Ratio of Multicarrier Modulation by Selected Mapping},
  Author                   = {R. W. Baaauml and R. F. H. Fisher and J. B. Huber},
  Journal                  = {Elect. Lett.},
  Year                     = {1996},

  Month                    = {Oct.},
  Number                   = {22},
  Pages                    = {2056-57},
  Volume                   = {32}
}

@Article{Benvenuto10,
  Title                    = {Single Carrier Modulation With Nonlinear Frequency Domain Equalization: An Idea Whose Time Has Come - Again},
  Author                   = {Benvenuto, N. and Dinis, R. and Falconer, D. and Tomasin, S.},
  Journal                  = {Proc. IEEE},
  Year                     = {2010},
  Number                   = {1},
  Pages                    = {69-96},
  Volume                   = {98}
}

@Article{OFDM,
  Title                    = {Multicarrier modulation for data transmission: An idea whose time has come},
  Author                   = {J. A. C. Bingham},
  Journal                  = { IEEE Commun. Mag.},
  Year                     = {1990},

  Month                    = {May },
  Number                   = {5},
  Pages                    = { 5-14},
  Volume                   = {28}
}

@Article{SLM32,
  Title                    = {SLM Peak-Power Reduction without Explicit Side Information},
  Author                   = {H. Breiling and S. H. Muuuller-Weinfurtner and J. B. Huber},
  Journal                  = {IEEE Commun. Lett.},
  Year                     = {2001},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {239-41},
  Volume                   = {5}
}

@Article{Canale13,
  Title                    = {Optimal Planning and Routing in Medium Voltage PowerLine Communications Networks},
  Author                   = {Canale, S. and Di Giorgio, A. and Lanna, A. and Mercurio, A. and Panfili, M. and Pietrabissa, A.},
  Journal                  = {IEEE Trans. Smart Grid},
  Year                     = {2013},

  Month                    = {Jun.},
  Number                   = {2},
  Pages                    = {711-719},
  Volume                   = {4}
}

@Article{Chan89,
  Title                    = {Amplitude, width, and interarrival distributions for noise impulses on intrabuilding power line communication networks},
  Author                   = {Chan, Morgan H L and Donaldson, R.W.},
  Journal                  = {IEEE Trans. Electromagn. Compat.},
  Year                     = {1989},

  Month                    = {Aug.},
  Number                   = {3},
  Pages                    = {320-323},
  Volume                   = {31}
}

@Article{Pend11004,
  Title                    = {{V}-{OFDM}: On Performance Limits over Multi-Path Rayleigh Fading Channels},
  Author                   = {P. Cheng and M. Tao and Y. Xiao and W. Zhang},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {2011},

  Month                    = {Jul.},
  Number                   = {7},
  Pages                    = {1878-1892},
  Volume                   = {59}
}

@Article{Smart_Grid13,
  Title                    = {Relay-Aided Amplify-and-Forward Powerline Communications},
  Author                   = {Cheng, X. and Cao, R. and Yang, L.},
  Journal                  = {IEEE Trans. Smart Grid},
  Year                     = {2013},

  Month                    = { },
  Number                   = {99},
  Pages                    = {1 -8},
  Volume                   = {PP}
}

@Article{9Cowley,
  Title                    = {{COFDM} tuner with impulse noise reduction},
  Author                   = {N. P. Cowley and A. Payne and M. Dawkins},
  Journal                  = {Eur. Patent Appl. EP1180851},
  Year                     = {Feb. 2002}
}

@Article{Crussiere06,
  Title                    = {Adaptive spread-spectrum multicarrier multiple-access over wirelines},
  Author                   = {Crussiere, M. and Baudais, J. and Helard, J.},
  Journal                  = {IEEE J. Sel. Areas in Commun.},
  Year                     = {2006},

  Month                    = {Jul.},
  Number                   = {7},
  Pages                    = {1377-1388},
  Volume                   = {24}
}

@InProceedings{Crussiere06_conf,
  Title                    = {Improved Throughput over Wirelines with Adaptive {MC-DS-CDMA}},
  Author                   = {Crussiere, M. and Baudais, J. and Helard, J. -F},
  Booktitle                = {Proc. IEEE Int. Symp. Spread Spectr. Techn. Appl.},
  Year                     = {2006},
  Month                    = {Aug.},
  Pages                    = {143-147}
}

@Article{2Cuntic,
  Title                    = {Analysis of Modulation Methods for Data Communications over the Low-voltage Grid},
  Author                   = {P. Cuntic and A. Baiant},
  Journal                  = {Proceeding of the 7th International Conference on Telecommunication ConTEL},
  Year                     = {2002},
  Pages                    = {20--23}
}

@Article{d2010power016,
  Title                    = {On power allocation in adaptive cyclic prefix {OFDM}},
  Author                   = {D Alessandro, Salvatore and Tonello, Andrea M and Lampe, Lutz},
  Journal                  = {in Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2010},

  Month                    = {Mar.},
  Pages                    = {183--188}
}

@Article{DaSilva94,
  Title                    = {Multicarrier orthogonal {CDMA} signals for quasi-synchronous communication systems},
  Author                   = {DaSilva, V.M. and Sousa, E.S.},
  Journal                  = {IEEE J. Sel. Areas in Commun.},
  Year                     = {1994},

  Month                    = {Jun.},
  Number                   = {5},
  Pages                    = {842-852},
  Volume                   = {12}
}

@Article{PAPR_coding_18,
  Title                    = {Peak-to-Mean Power Control in {OFDM}, Golay Complementary Sequences, and Reed-Muller Codes},
  Author                   = {J. A. Davis and J. Jedwab},
  Journal                  = { IEEE Trans. Info. Theory},
  Year                     = {1999},

  Month                    = {Nov.},
  Number                   = {7},
  Pages                    = {2397-17},
  Volume                   = {45}
}

@Article{Del03,
  Title                    = {Comparison of {CDMA} and {OFDM} techniques for downstream power-line communications on low voltage grid},
  Author                   = {Del Re, E. and Fantacci, R. and Morosi, S. and Seravalle, R.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2003},

  Month                    = {Oct.},
  Number                   = {4},
  Pages                    = {1104-1109},
  Volume                   = {18}
}

@Article{Fantacci03,
  Title                    = {Comparison of {CDMA} and {OFDM} techniques for downstream power-line communications on low voltage grid},
  Author                   = {Del Re, E. and Fantacci, R. and Morosi, S. and Seravalle, R.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2003},

  Month                    = {Oct.},
  Number                   = {4},
  Pages                    = {1104-1109},
  Volume                   = {18}
}

@Article{PD_3,
  Title                    = {Comparison of {CDMA} and {OFDM} techniques for downstream power-line communications on low voltage grid},
  Author                   = {Del Re, E. and Fantacci, R. and Morosi, S. and Seravalle, R.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2003},

  Month                    = {Oct.},
  Number                   = {4},
  Pages                    = { 1104-1109},
  Volume                   = {18}
}

@Article{Re03,
  Title                    = {Comparison of {CDMA} and {OFDM} techniques for downstream power-line communications on low voltage grid},
  Author                   = {Del Re, E. and Fantacci, R. and Morosi, S. and Seravalle, R.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2003},

  Month                    = {Oct.},
  Number                   = {4},
  Pages                    = {1104-1109},
  Volume                   = {18}
}

@InProceedings{Bert13,
  Title                    = {{MAC} enhancements for {G3-PLC} home networks},
  Author                   = {Di Bert, L. and D'Alessandro, S. and Tonello, AM.},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2013},
  Month                    = {Mar.},
  Pages                    = {155-160}
}

@Article{1Esmailian,
  Title                    = {An In-Building Power Line Channel Simulator},
  Author                   = {T. Esmailian and F. R. Kschischang and P. G. Gulak},
  Journal                  = {Proceedings of the International Symposium on Power Line Communication and its Applications},
  Year                     = {2002},
  Pages                    = {2-3}
}

@InProceedings{Fairel95,
  Title                    = {A flexible and high performance cellular mobile cornrnunications system based on orthogonal multicarrier {SSMA}},
  Author                   = {K. Fairel and S. Kaiser and M. Schnell},
  Booktitle                = {Wireless Pers. Commun.},
  Year                     = {1995},
  Pages                    = {121-144},
  Volume                   = {2}
}

@Article{Galli03,
  Title                    = {Broadband is power: internet access through the power line network},
  Author                   = {Galli, S. and Scaglione, A. and Dostert, K.},
  Journal                  = {IEEE Commun. Mag.},
  Year                     = {2003},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {82-83},
  Volume                   = {41}
}

@Article{Galli11,
  Title                    = {For the Grid and Through the Grid: The Role of Power Line Communications in the Smart Grid},
  Author                   = {Galli, S. and Scaglione, A. and Zhifang Wang},
  Journal                  = {Proc. IEEE},
  Year                     = {2011},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {998-1027},
  Volume                   = {99}
}

@Article{Ghosh96022,
  Title                    = {Analysis of the effect of impulse noise on multicarrier and single carrier {QAM} systems},
  Author                   = {M. Ghosh},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {1996},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {145-147},
  Volume                   = {44}
}

@Article{PAPR_coding_16,
  Title                    = {Complementary Series},
  Author                   = {M. Golay},
  Journal                  = {IEEE Trans. Info. Theory},
  Year                     = {1961},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {82-87},
  Volume                   = {7}
}

@Book{Goldsmith05,
  Title                    = {Wireless Communications},
  Author                   = {A Goldsmith},
  Publisher                = {Cambridge University Press},
  Year                     = {2005}
}

@Article{SP_magazine04,
  Title                    = {Power line channel characteristics and their effect on communication system design},
  Author                   = {Gotz, M. and Rapp, M. and Dostert, K.},
  Journal                  = {IEEE Commun. Mag.},
  Year                     = {2004},

  Month                    = {Apr.},
  Number                   = {4},
  Pages                    = {78-86},
  Volume                   = {42}
}

@Article{han2010constellation005,
  Title                    = {Constellation-rotated vector {OFDM} and its performance analysis over {R}ayleigh fading channels},
  Author                   = {Han, Chenggao and Hashimoto, Takeshi and Suehiro, Naoki},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {2010},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {828--838},
  Volume                   = {58}
}

@Article{Hara97,
  Title                    = {Overview of Multicarrier {CDMA}},
  Author                   = {S. Hara and R. Prasad},
  Journal                  = {IEEE Commun. Mag.},
  Year                     = {Dec. 1997},
  Number                   = {12},
  Pages                    = {126-133},
  Volume                   = {35}
}

@Article{Zhidkov2006_19,
  Title                    = {Iterative decoding of codes over complex numbers for impulsive noise channels},
  Author                   = {J. Haring and A. J. Han Vinck },
  Journal                  = { IEEE Trans. Inf. Theory},
  Year                     = {2003},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {1251-1260},
  Volume                   = {49}
}

@Article{Hadamard70,
  Title                    = {Transmission of Information by Orthogonal Functions},
  Author                   = {H.F. Harmuth},
  Journal                  = {Springer-Verlag, Berlin},
  Year                     = {1970}
}

@Article{Hazen08,
  Title                    = {The Technology Behind {H}ome{P}lug {AV} Powerline Communications},
  Author                   = {Hazen, M.E.},
  Journal                  = {Computer},
  Year                     = {2008},
  Number                   = {6},
  Pages                    = {90-92},
  Volume                   = {41}
}

@Article{Hazen2008,
  Title                    = {The Technology Behind HomePlug {AV} Powerline Communications},
  Author                   = {Hazen, M.E.},
  Journal                  = {Computer},
  Year                     = {2008},
  Number                   = {6},
  Pages                    = {90-92},
  Volume                   = {41}
}

@Article{Heylieri06,
  Title                    = {Power Line Communications ({G}uest {E}ditorial)},
  Author                   = {Heylieri, E. and Galli, S. and Lee, Y. W. and Poor, H. and Vinvk, H.},
  Journal                  = {IEEE J. Sel. Areas Commun.},
  Year                     = {2006},

  Month                    = {Jul.},
  Number                   = {7},
  Pages                    = {1261-1266},
  Volume                   = {24}
}

@Article{Hooijen98,
  Title                    = {{A} channel model for the residential power circuit used as a digital communications medium},
  Author                   = {Hooijen, O.G.},
  Journal                  = {IEEE Trans. Electromagn. Compat.},
  Year                     = {1998},
  Number                   = {4},
  Pages                    = {331-336},
  Volume                   = {40}
}

@Article{huang2011minimal013,
  Title                    = {Minimal Euclidean distance-inspired optimal and suboptimal modulation schemes for vector {OFDM} system},
  Author                   = {Huang, Xin-Lin and Wang, Gang and Hu, Fei},
  Journal                  = {Int. J. Commun. Syst.},
  Year                     = {2011},

  Month                    = {Aug.},
  Number                   = {5},
  Pages                    = {553-567},
  Volume                   = {24},

  Publisher                = {Wiley Online Library}
}

@Article{Zhidkov2006_14,
  Title                    = {Performance of the locally optimum threshold receiver and several suboptimal nonlinear receivers for {ELF} noise},
  Author                   = {R. Ingram},
  Journal                  = {IEEE J Ocean. Eng.},
  Year                     = {1984},

  Month                    = {Jul.},
  Number                   = {3},
  Pages                    = { 202-208},
  Volume                   = {OE-9}
}

@InProceedings{Jasbi13,
  Title                    = {Hybrid Overlay/Underlay {MC-CDMA} for Cognitive Radio Networks with {MMSE} Channel Equalization},
  Author                   = {Jasbi, F. and So, D. K. C. and Alsusa, Emad},
  Booktitle                = {Proc. IEEE GLOBECOM},
  Year                     = {Sept. 2013}
}

@InProceedings{Jayalath02,
  Title                    = {A blind {SLM} receiver for {PAR}-reduced {OFDM}},
  Author                   = {Jayalath, A. D S and Tellambura, C.},
  Booktitle                = {Proc. IEEE Veh. Technol. Conf.},
  Year                     = {Sep. 2002},
  Pages                    = {219-222},
  Volume                   = {1}
}

@InProceedings{Jianming11,
  Title                    = {Communication performance of broadband {PLC} technologies for smart grid},
  Author                   = {Liu Jianming and Zhao Bingzhen and Geng Liang and Yuan Zhou and Wang Yirong},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2011},
  Month                    = {Apr.},
  Pages                    = {491-496}
}

@Article{PAPR_coding_13,
  Title                    = {Block Coding Scheme for Reduction of Peak to Mean Envelope Power Ratio of Multicarrier Transmission Scheme},
  Author                   = {A. E. Jones and T. A. Wilkinson and S. K. Barton},
  Journal                  = { Elect. Lett.},
  Year                     = {1994},

  Month                    = {Dec.},
  Number                   = {22},
  Pages                    = {2098-99},
  Volume                   = {30}
}

@Article{joung2014spectral018,
  Title                    = {Spectral efficiency and energy efficiency of {OFDM} systems: Impact of power amplifiers and countermeasures},
  Author                   = {Joung, Jingon and Ho, Chin Keong and Sun, Sumei},
  Journal                  = {IEEE J. Sel. Areas Commun.},
  Year                     = {2014},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {208--220},
  Volume                   = {32}
}

@Article{Katayama06,
  Title                    = {A mathematical model of noise in narrowband power line communication systems},
  Author                   = {Katayama, M. and Yamazato, T. and Okada, H.},
  Journal                  = {IEEE J. Sel. Areas in Commun.},
  Year                     = {2006},

  Month                    = {Jul.},
  Number                   = {7},
  Pages                    = {1267-1276},
  Volume                   = {24}
}

@InProceedings{Katsis03,
  Title                    = {Coded {MC-CDMA} systems for power line communications},
  Author                   = {Katsis, P.L. and Papadopoulos, G.D. and PavJidou, F.-N.},
  Booktitle                = {Proc. of Int. Conf. on Telecommun. in Modern Satellite, Cable and Broadcasting Service},
  Year                     = {2003},
  Month                    = {Oct.},
  Pages                    = {153-156},
  Volume                   = {1}
}

@InProceedings{Kim10,
  Title                    = {Performance Analysis and Enhancements of Narrowband {OFDM} Powerline Communication Systems},
  Author                   = {Il Kim and Varadarajan, B. and Dabak, A},
  Booktitle                = {Proc. IEEE Int. Conf. Smart Grid Commun. (SmartGridComm)},
  Year                     = {2010},
  Month                    = {Oct.},
  Pages                    = {362-367}
}

@Article{Kim99,
  Title                    = {A multicarrier {CDMA} system with adaptive subchannel allocation for forward links},
  Author                   = {Yun Hee Kim and Iickho Song and Seokho Yoon and So Ryoung Park},
  Journal                  = {IEEE Trans. Veh. Technol.},
  Year                     = {1999},

  Month                    = {Sept.},
  Number                   = {5},
  Pages                    = {1428-1436},
  Volume                   = {48}
}

@Article{Kirlin76,
  Title                    = {Pseudo-random analog noise generation},
  Author                   = {Kirlin, R.L.},
  Journal                  = {Proc. IEEE},
  Year                     = {1976},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {824-826},
  Volume                   = {64}
}

@InProceedings{Kondo93,
  Title                    = {On the use of multicarrier direct sequence spread spectrum systems},
  Author                   = {Kondo, S. and Milstein, L.B.},
  Booktitle                = {Proc. IEEE Milcom.},
  Year                     = {1993},
  Month                    = {Oct.},
  Pages                    = {52-56},
  Volume                   = {1}
}

@Article{Lai12,
  Title                    = {Using the Wireless and {PLC} Channels for Diversity},
  Author                   = {Lai, S.W. and Messier, G.G.},
  Journal                  = {IEEE Trans. Commun},
  Year                     = {2012},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {3865-3875},
  Volume                   = {60}
}

@InProceedings{Lampe12,
  Title                    = {Cooperative multihop power line communications},
  Author                   = {L. Lampe and A. J. H. Vinck},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2012},
  Month                    = {Mar.},
  Pages                    = {1-6},

  Doi                      = {10.1109/ISPLC.2012.6201337},
  ISSN                     = {PENDING},
  Keywords                 = {carrier transmission on power lines;cooperative communication;data communication;PLC networks;communication signals;cooperative multihop power line communications;data communication;diversity advantage;end-to-end transmission rate;multihop transmission;power line networks;wireless domain;wireless transmission;Automatic repeat request;Power cables;Relays;Signal to noise ratio;Spread spectrum communication;Transfer functions;Wireless communication}
}

@InProceedings{4913423020,
  Title                    = {Performance of scaled {SLM} for {PAPR} reduction of {OFDM} signal in {PLC} channels},
  Author                   = {J. S. Lee and H. M. Oh and J. T. Kim and J. Y. Kim},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2009},
  Month                    = {Mar.},
  Pages                    = {166-170}
}

@Article{Clipping_1998,
  Title                    = {Effects of clipping and filtering on the performance of OFDM},
  Author                   = {X. Li and L. J. Cimini Jr.},
  Journal                  = {IEEE Commun. Lett.},
  Year                     = {1998},

  Month                    = {May },
  Pages                    = {131-133},
  Volume                   = {2}
}

@Article{PAPR_clippingFiltering11,
  Title                    = {Effect of Clipping and Filtering on the Performance of OFDM},
  Author                   = {X. Li and L. J. Cimini, Jr.},
  Journal                  = {IEEE Commun. Lett.},
  Year                     = {1998},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {131-33},
  Volume                   = {2}
}

@Article{li2012performance001,
  Title                    = {On performance of vector {OFDM} with linear receivers},
  Author                   = {Li, Yabo and Ngebani, Ibo and Xia, Xiang-Gen and H{\o}st-Madsen, Anders},
  Journal                  = {IEEE Trans. Signal Process.},
  Year                     = {2012},

  Month                    = {Nov.},
  Number                   = {10},
  Pages                    = {5268--5280},
  Volume                   = {60}
}

@InProceedings{Liu09,
  Title                    = {Experience of {AMR} systems based on {BPL} in China},
  Author                   = {Qingyang Liu and Bingzhen Zhao and Yirong Wang and Jing Hu},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2009},
  Month                    = {Mar.},
  Pages                    = {280-284}
}

@Article{Wenqing11,
  Title                    = {Channel characterization and system verification for narrowband power line communication in smart grid applications},
  Author                   = {Wenqing Liu and Sigle, M. and Dostert, K.},
  Journal                  = {IEEE Commun. Mag.},
  Year                     = {2011},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {28-35},
  Volume                   = {49}
}

@Article{Crussiere07,
  Title                    = {Resource allocation with adaptive spread spectrum {OFDM} using 2{D} spreading for power line communications},
  Author                   = {J.-Y. Baudais et M. Crussière},
  Journal                  = { EURASIP J. Advances Signal Process.},
  Year                     = {2007},
  Pages                    = {1-13},
  Volume                   = {2007}
}

@Article{PD_4,
  Title                    = {Performance analysis of OFDM systems for broadband power line communications under impulsive noise and multipath effects},
  Author                   = {Ma, Y.H. and So, P.L. and Gunawan, E.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2005},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = { 674-682},
  Volume                   = {20}
}

@Article{Ma08,
  Title                    = {Comparison of {CDMA} and {OFDM} Systems for Broadband Power Line Communications},
  Author                   = {Ma, Y. H. and So, P.L. and Gunawan, E.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2008},

  Month                    = {Oct.},
  Number                   = {4},
  Pages                    = {1876-1885},
  Volume                   = {23}
}

@Article{So05,
  Title                    = {Performance analysis of {OFDM}
system for broadband power line communications under impulsive noise and multipath effects},
  Author                   = {Y. H. Ma and P. L. So and E. Gunawan },
  Journal                  = { IEEE Trans. Power Del.},
  Year                     = {2005},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {674-682},
  Volume                   = {20}
}

@Article{Matanza13,
  Title                    = {Difference sets-based compressive sensing as denoising method for narrow-band power line communications},
  Author                   = {Matanza, J. and Alexandres, S. and Rodriguez-Morcillo, C.},
  Journal                  = {IET Commun.},
  Year                     = {2013},

  Month                    = {Oct.},
  Number                   = {15},
  Pages                    = {1580-1586},
  Volume                   = {7}
}

@Article{PD_1,
  Title                    = {Modeling and analysis of noise effects on broadband power-line communications},
  Author                   = {H. Meng and Y. L. Guan and S. Chen},
  Journal                  = { IEEE Trans. Power Del.},
  Year                     = {2005},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = { 630-637},
  Volume                   = {20}
}

@Article{Middleton83,
  Title                    = {Canonical and quasi-canonical probability models of class {A} interference},
  Author                   = {D. Middleton},
  Journal                  = {IEEE Trans. Electromagn. Compat.},
  Year                     = {May 1983},
  Pages                    = {76-106},
  Volume                   = { EMC-25}
}

@Article{Middleton77,
  Title                    = {Statistical-physical models of electromagnetic interference},
  Author                   = {D. Middleton},
  Journal                  = {IEEE Trans. Electromagn. Compat.},
  Year                     = {Aug. 1977},
  Pages                    = {106-127},
  Volume                   = { EMC-19}
}

@Article{Zhidkov2003_8,
  Title                    = {Non-Gaussian noise models in signal processing for telecommunications: new methods an results for class-{A} and class-{B} noise models},
  Author                   = {Middleton, D.},
  Journal                  = {IEEE Trans. Inform. Theory},
  Year                     = {1999},

  Month                    = {May},
  Number                   = {4},
  Pages                    = {1129 -1149},
  Volume                   = {45}
}

@Article{Middleton72,
  Title                    = {Statistical-Physical Models of Urban Radio-Noise Environments - Part {I}: Foundations},
  Author                   = {Middleton, D.},
  Journal                  = {IEEE Trans. Electromagn. Compat.},
  Year                     = {1972},

  Month                    = {May},
  Number                   = {2},
  Pages                    = {38-56},
  Volume                   = {EMC-14}
}

@InProceedings{Mudriievskyi13,
  Title                    = {{CSMA/CA}: Improvements of the contention window adaptation},
  Author                   = {Mudriievskyi, S. and Radeke, R. and Lehnert, R.},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2013},
  Month                    = {Mar.},
  Pages                    = {53-57}
}

@Article{Muller1997,
  Title                    = {OFDM with Reduced Peak-to-Average Power Ratio by Optimum Combination of Partial Transmit Sequences},
  Author                   = {S. H. Muller and J. B. Huber},
  Journal                  = { Elect. Lett.},
  Year                     = {1997},

  Month                    = {Feb.},
  Number                   = {5},
  Pages                    = {368-69},
  Volume                   = {33}
}

@Article{Muller97,
  Title                    = {{OFDM} with Reduced Peak-to-Average Power Ratio by Optimum Combination of Partial Transmit Sequences},
  Author                   = {S. H. Muller and J. B. Huber},
  Journal                  = { Elect. Lett.},
  Year                     = {1997},

  Month                    = {Feb.},
  Number                   = {5},
  Pages                    = {368-69},
  Volume                   = {33}
}

@Article{SLM30,
  Title                    = {A Comparison of Peak Power Reduction Schemes for OFDM},
  Author                   = {S. H. Muuuller and J. B. Huber},
  Journal                  = {Proc. IEEE GLOBECOM '97},
  Year                     = {1997},

  Month                    = {Nov.},
  Pages                    = {1-5}
}

@Article{Goodman06,
  Title                    = {{S}ingle carrier {FDMA} for uplink wireless transmission},
  Author                   = {Myung, H.G. and Junsung Lim and Goodman, D.},
  Journal                  = {IEEE Veh. Technol. mag.},
  Year                     = {2006},
  Number                   = {3},
  Pages                    = {30-38},
  Volume                   = {1}
}

@InProceedings{Nassar12b,
  Title                    = {Cyclostationary noise modeling in narrowband powerline communication for Smart Grid applications},
  Author                   = {Nassar, M. and Dabak, A and Il Han Kim and Pande, T. and Evans, B.L.},
  Booktitle                = {Proc. IEEE Int. Conf. Acoustics, Speech and Signal Process. (ICASSP)},
  Year                     = {2012},
  Month                    = {Mar.},
  Pages                    = {3089-3092}
}

@Article{Nassar12,
  Title                    = {Local Utility Power Line Communications in the 3-500 kHz Band: Channel Impairments, Noise, and Standards},
  Author                   = {Nassar, M. and Jing Lin and Mortazavi, Y. and Dabak, A and Il Han Kim and Evans, B.L.},
  Journal                  = {IEEE Signal Process. Mag.},
  Year                     = {2012},

  Month                    = {Sept.},
  Number                   = {5},
  Pages                    = {116-127},
  Volume                   = {29}
}

@Article{Book_CCDF,
  Title                    = {{OFDM} for Wireless Multimedia Communications},
  Author                   = {R. van Nee and R. Prasad},
  Journal                  = {Artech House},
  Year                     = {2000}
}

@InProceedings{ngebani2013analysis007,
  Title                    = {Analysis of phase noise in vector {OFDM} systems},
  Author                   = {Ngebani, Ibo and Li, Yabo and Xia, Xiang-Gen and Ahmed, Haider Sami and Zhao, Minjian},
  Booktitle                = {Proc.IEEE Global Communications Conference (GLOBECOM), 2013},
  Year                     = {2013},
  Month                    = {Dec.},
  Pages                    = {3602--3607}
}

@Article{Ibo16003,
  Title                    = {{EM}-Based Phase Noise Estimation in Vector {OFDM} Systems Using Linear {MMSE} Receivers},
  Author                   = {I. Ngebani and Yabo Li and Xiang-Gen Xia and Minjian Zhao},
  Journal                  = {IEEE Trans. Veh. Technol.},
  Year                     = {2016},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {110-122},
  Volume                   = {65}
}

@Article{Nguyen08,
  Title                    = {Bit-Interleaved Coded {OFDM} With Iterative Decoding in Impulsive Noise},
  Author                   = {Nguyen, H.H. and Bui, T.Q.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2008},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {640-649},
  Volume                   = {23}
}

@Article{nguyen2008partial015,
  Title                    = {On partial transmit sequences for {PAR} reduction in {OFDM} systems},
  Author                   = {Nguyen, Trung Thanh and Lampe, Lutz},
  Journal                  = {IEEE Trans. Wireless Commun.},
  Year                     = {2008},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {746--755},
  Volume                   = {7}
}

@InProceedings{Nikfar14,
  Title                    = {{MIMO} capacity of class {A} impulsive noise channel for different levels of information availability at transmitter},
  Author                   = {Nikfar, B. and Akbudak, T. and Vinck, AJ.H.},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun. and its Appl. (ISPLC)},
  Year                     = {2014},
  Month                    = {Mar.},
  Pages                    = {266-271}
}

@Article{PAPR_clipping10,
  Title                    = {Envelope Variations and Spectral Splatter in Clipped Multicarrier Signals},
  Author                   = {R. O'Neill and L. B. Lopes},
  Journal                  = {Proc. IEEE PIMRC '95},
  Year                     = {1995},

  Month                    = {Toronto, Canada, Sept.},
  Pages                    = {71-75}
}

@Article{PAPR_Ochiai01,
  Title                    = {On the distribution of the peak-to-average power ratio in {OFDM} signals},
  Author                   = {Ochiai, H. and Imai, H.},
  Journal                  = { IEEE Trans. Commun.},
  Year                     = {2001},
  Number                   = {2},
  Pages                    = {282-289},
  Volume                   = {49}
}

@InProceedings{Oh06,
  Title                    = {Mitigation of Performance Degradation by Impulsive Noise in {LDPC} Coded {OFDM} System},
  Author                   = {Hui-Myoung Oh and Young-Jin Park and Sungsoo Choi and Jae-Jo Lee and Keum-Chan Whang},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2006},
  Pages                    = {331-336}
}

@InProceedings{Ohkubo03,
  Title                    = {Design criteria for phase sequences in selected mapping},
  Author                   = {Ohkubo, N. and Ohtsuki, T.},
  Booktitle                = {Proc. IEEE Veh. Technol. Conf. (VTC)},
  Year                     = {2003},
  Month                    = {Apr.},
  Pages                    = {373-377},
  Volume                   = {1}
}

@InProceedings{Ohkubo02,
  Title                    = {A peak to average power ratio reduction of multicarrier {CDMA} using selected mapping},
  Author                   = {Ohkubo, N. and Ohtsuki, T.},
  Booktitle                = {Proc. IEEE Veh. Technol. Conf. (VTC)},
  Year                     = {2002},
  Pages                    = {2086-2090},
  Volume                   = {4}
}

@Article{Oppenmann97,
  Title                    = {Orthogonal complex-valued spreading sequences with a wide range of correlation properties},
  Author                   = {I. Oppenmann},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {1997},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {1379-1380},
  Volume                   = {45}
}

@Article{Pavlidou03,
  Title                    = {Power line communications: state of the art and future trends},
  Author                   = {Pavlidou, N. and Vinck, A.J.H. and Yazdani, J. and Honary, B.},
  Journal                  = {IEEE Commun. Mag.},
  Year                     = {2003},

  Month                    = {Apr.},
  Number                   = {4},
  Pages                    = {34-40},
  Volume                   = {41}
}

@Article{3Philipps,
  Title                    = {Development of a Statistical Model for Powerline Communication Channels},
  Author                   = {H. Philipps},
  Journal                  = {International Symposium on Power Line Communications (ISPLC)},
  Year                     = {2000},

  Month                    = {Apr.},
  Pages                    = {153-160}
}

@Book{Proakis01,
  Title                    = {Digital Communications},
  Author                   = {J. Proakis},
  Publisher                = {4th ed. New York: McGraw-Hill},
  Year                     = {2001}
}

@Article{Emad_Khaled13_2,
  Title                    = {Quantized Peak-Based Impulsive Noise Blanking in Power-Line Communications},
  Author                   = {Rabie, K.M. and Alsusa, E.},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {Feb. 2014},
  Number                   = {99},
  Pages                    = {1-1},
  Volume                   = {PP}
}

@Article{Emad_Khaled13_3,
  Title                    = {Preprocessing Based Impulsive Noise Reduction for Power-Line Communications},
  Author                   = {K. Rabie and E. Alsusa},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2014},

  Month                    = {Aug.},
  Number                   = {4},
  Pages                    = {1648-1658},
  Volume                   = {29}
}

@InProceedings{rabie2015constant009,
  Title                    = {Constant envelope {OFDM} transmission over impulsive noise power-line communication channels},
  Author                   = {Rabie, KM and Alsusa, E and Familua, AD and Cheng, L},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {2015},
  Month                    = {Mar.},
  Pages                    = {13-18}
}

@InProceedings{RabieISPLC16,
  Title                    = {Improving Energy Efficiency in Dual-hop Cooperative {PLC} Relaying Systems},
  Author                   = {Rabie, K. M. and Adebisi, B. and Salem, A.},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun. and its Appl. (ISPLC)},
  Year                     = {2016},
  Pages                    = {196-200},
  month                    = {Mar.}
}

@Article{Rabie_Preprocessing,
  Title                    = {Preprocessing-Based Impulsive Noise Reduction for Power-Line Communications},
  Author                   = {K. M. Rabie and E. Alsusa},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2014},

  Month                    = {Aug},
  Number                   = {4},
  Pages                    = {1648-1658},
  Volume                   = {29}
}

@InProceedings{rabie2013efficient010,
  Title                    = {Efficient {SLM} based impulsive noise reduction in powerline {OFDM} communication systems},
  Author                   = {Rabie, Khaled M and Alsusa, Emad},
  Booktitle                = {Proc. IEEE Global Commun. Conf. (GLOBECOM)},
  Year                     = {2013},
  Month                    = {Dec.},
  Pages                    = {2915--2920}
}

@InProceedings{Raphaeli99,
  Title                    = {A comparison between {OFDM}, single carrier and spread for high data rate {PLC}},
  Author                   = {D. Rabphaeli and E. Bassin},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {Mar. 1999}
}

@InProceedings{1433806019,
  Title                    = {Adaptive technique for impulsive noise cancellation in broad-band power line communication system},
  Author                   = {F. Rouissi and F. Tlili and A. Ghazel and A. Zeddam},
  Booktitle                = {Proc. IEEE Int. Symp. Signal Process. Inf. Technol. (ISSPIT)},
  Year                     = {2004},
  Month                    = {Dec.},
  Pages                    = {413-416}
}

@Article{Zhidkov2003_11,
  Title                    = {Impulsive noise measurements and characterization in a {UHF} digital {TV} channel},
  Author                   = {M. G. Sanchez and L. de Haro and M. C. Ramon and A. Mansilla and C. M. Ortega and D. Oliver},
  Journal                  = {IEEE Trans. Electromagn. Compat.},
  Year                     = {1999},

  Month                    = {May},
  Number                   = {2},
  Pages                    = {124 -136},
  Volume                   = {41}
}

@InProceedings{Schulz00012,
  Title                    = {Comparison of {CDMA} and {OFDM} for data communications on the medium voltage power grid},
  Author                   = {W. Schulz and S. Schwarze},
  Booktitle                = {Proc. IEEE Int. Symp. Power Lines Commun.  and its Appl. (ISPLC)},
  Year                     = {Apr. 2000}
}

@Article{Zhidkov2006_15,
  Title                    = {Locally optimum and suboptimum detector performance in a non-Gaussian interference environment},
  Author                   = {A. D. Spaulding},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {1985},

  Month                    = {Jun. },
  Pages                    = {509-517},
  Volume                   = {COM-33}
}

@Article{PAPR_coding_15,
  Title                    = {On the Computation and Reduction of the Peak-to-Average Power Ratio in Multicarrier Communications},
  Author                   = {V. Tarokh and H. Jafarkhani},
  Journal                  = { IEEE Trans. Commun.},
  Year                     = {2000},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {37-44},
  Volume                   = {48}
}

@Article{Tarokh00,
  Title                    = {On the computation and reduction of the peak-to-average power ratio in multicarrier communications},
  Author                   = {Tarokh, Vahid and Jafarkhani, Hamid},
  Journal                  = {IEEE Trans. commun.},
  Year                     = {2000},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {37-44},
  Volume                   = {48}
}

@Article{PAPR_TR22,
  Title                    = {Peak to Average Power Reduction for Multicarrier Modulation},
  Author                   = {J. Tellado},
  Journal                  = {Ph.D. dissertation},
  Year                     = {2000},

  Month                    = { Stanford Univ.}
}

@Book{Tellado00,
  Title                    = {Multicarrier Modulation With Low {PAR}: Applications to {DSL} and Wireless},
  Author                   = {J. Tellado},
  Publisher                = {Norwell, MA: Kluwer},
  Year                     = {2000}
}

@InProceedings{Tonello10Globecom,
  Title                    = {Opportunistic Relaying in In-Home {PLC} Networks},
  Author                   = {A. M. Tonello and F. Versolatto and S. D'Alessandro},
  Booktitle                = {Proc. IEEE Global Telecommun. Conf. (GLOBECOM)},
  Year                     = {2010},
  Month                    = {Dec.},
  Pages                    = {1-5},

  Doi                      = {10.1109/GLOCOM.2010.5683175},
  ISSN                     = {1930-529X},
  Keywords                 = {carrier transmission on power lines;channel capacity;decode and forward communication;statistical analysis;telecommunication network topology;time division multiple access;transfer functions;transmission line theory;channel transfer function;decode and forward scheme;in-home PLC networks;in-home power line communication networks;network capacity;opportunistic relaying;optimal time slot duration;statistical topology model;time division multiple access;transmission line theory;Attenuation;Modems;Network topology;Protocols;Relays;Time division multiple access;Topology}
}

@Article{Tonello14Comms,
  Title                    = {In-Home Power Line Communication Channel: Statistical Characterization},
  Author                   = {A. M. Tonello and F. Versolatto and A. Pittolo},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {2014},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {2096-2106},
  Volume                   = {62},

  Doi                      = {10.1109/TCOMM.2014.2317790},
  ISSN                     = {0090-6778},
  Keywords                 = {carrier transmission on power lines;coherence;frequency response;indoor communication;statistical analysis;telecommunication channels;CFR;PLC channel;average channel gain;channel frequency response;closed-form expressions;coherence bandwidth;frequency 1.8 MHz to 100 MHz;in-home power line communications;line impedance;receiver outlet;root-mean-square delay spread;statistical characterization;transmitter outlet;Correlation;Delays;Frequency measurement;Impedance;Receivers;Standards;Transmitters;Power line communications (PLC) channel;broadband PLC;channel characterization;fading;spatial correlation}
}

@InProceedings{Tunc13,
  Title                    = {Pilot based channel estimation and transform domain analysis in broadband {PLC} for Smart Grid},
  Author                   = {Tunc, M.A. and Perrins, E.},
  Booktitle                = {Proc. IEEE Int. Conf. Smart Grid Commun. ({S}mart{G}rid{C}omm)},
  Year                     = {2013},
  Month                    = {Oct.},
  Pages                    = {283-288}
}

@InProceedings{6102311,
  Title                    = {The effect of LPTV channel adaptation on the performance of broadband PLC for Smart Grid},
  Author                   = {Tunc, M.A. and Perrins, E. and Lampe, L.},
  Booktitle                = {Smart Grid Communications (SmartGridComm), 2011 IEEE International Conference on},
  Year                     = {2011},
  Month                    = {Oct.},
  Pages                    = {167-171}
}

@InProceedings{Umehara04,
  Title                    = {Turbo decoding in impulsive noise environment},
  Author                   = {Umehara, D. and Yamaguchi, H. and Morihiro, Y.},
  Booktitle                = {Proc. IEEE Global Telecommun. Conf. (GLOBECOM)},
  Year                     = {2004},
  Month                    = {Nov.},
  Pages                    = {194-198},
  Volume                   = {1}
}

@Article{Zhidkov2006_13,
  Title                    = {Threshold detection in narrow-band non-Gaussian noise},
  Author                   = {K. S. Vastola },
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {1984},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {134-139},
  Volume                   = { COM-32}
}

@Article{Viterbi90,
  Title                    = {Very low rate convolution codes for maximum theoretical performance of spread-spectrum multiple-access channels},
  Author                   = {Viterbi, A.J.},
  Journal                  = {IEEE J. Sel. Areas in Commun.},
  Year                     = {1990},

  Month                    = {May},
  Number                   = {4},
  Pages                    = {641-649},
  Volume                   = {8}
}

@Article{Wang10,
  Title                    = {A Low-Complexity {PAPR} Estimation Scheme for {OFDM} Signals and Its Application to {SLM}-Based {PAPR} Reduction},
  Author                   = {Chin-Liang Wang and Sheng-Ju Ku and Chun-Ju Yang},
  Journal                  = {IEEE J. Sel. Topics Signal Process.},
  Year                     = {2010},

  Month                    = {Apr.},
  Number                   = {3},
  Pages                    = {637-645},
  Volume                   = {4}
}

@Article{weinstein1971data017,
  Title                    = {Data transmission by frequency-division multiplexing using the discrete {F}ourier transform},
  Author                   = {Weinstein, Stephen B and Ebert, Paul M},
  Journal                  = {IEEE Trans. Commun. Tech.},
  Year                     = {1971},

  Month                    = {Oct.},
  Number                   = {5},
  Pages                    = {628--634},
  Volume                   = {19}
}

@Article{Xia002,
  Title                    = {Precoded and vector {OFDM} robust to channel spectral nulls and with reduced cyclic prefix length in single transmit antenna systems},
  Author                   = {Xiang-Gen Xia},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {2001},

  Month                    = {Aug.},
  Number                   = {8},
  Pages                    = {1363-1374},
  Volume                   = {49}
}

@InProceedings{Yee93,
  Title                    = {Multi-Carrier {CDMA} in Indoor Wireless Radio Networks},
  Author                   = {N. Yee and J. P. Linnartz and G. Fettweis},
  Booktitle                = {Proc. IEEE Pers. Indoor and Mobile Radio Commun. (PIMRC)},
  Year                     = {Sept. 1993},
  Pages                    = {109-113}
}

@Article{Yoo11,
  Title                    = {Amplitude {PDF} Analysis of {OFDM} Signal Using Probabilistic {PAPR} Reduction Method},
  Author                   = {Hyunseuk Yoo and Frédéric Guilloud and Ramesh Pyndiah},
  Journal                  = {EURASIP Journal on Wireless Communications and Networking},
  Year                     = {2011},
  Volume                   = {2011}
}

@Article{Zhai11,
  Title                    = {Transmission Characteristics of Low-Voltage Distribution Networks in China Under the Smart Grids Environment},
  Author                   = {Ming-Yue Zhai},
  Journal                  = {IEEE Trans. Power Del.},
  Year                     = {2011},

  Month                    = {jan. },
  Number                   = {1},
  Pages                    = {173 -180},
  Volume                   = {26}
}

@Article{Zhidkov2008,
  Title                    = {Analysis and comparison of several simple impulsive noise mitigation schemes for {OFDM} receivers},
  Author                   = {S. V. Zhidkov},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {2008},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {5-9},
  Volume                   = {56}
}

@InProceedings{Zhidkov2004,
  Title                    = {On the analysis of {OFDM} receiver with blanking nonlinearity in impulsive noise channels},
  Author                   = {S. V. Zhidkov},
  Booktitle                = {Proc. Int. Symp. Intell. Signal Process. Commun. Syst.},
  Year                     = {2004},
  Month                    = {Nov.},
  Pages                    = {492-496}
}

@Article{Zhidkov03,
  Title                    = {Impulsive noise suppression in OFDM-based communication systems},
  Author                   = {S. V. Zhidkov},
  Journal                  = {IEEE Trans. Consum. Electron.},
  Year                     = {2003},

  Month                    = {Nov.},
  Number                   = {4},
  Pages                    = {944-948},
  Volume                   = {49}
}

@Article{Zhidkov2006_20,
  Title                    = {Impulsive noise suppression in OFDM-based communication systems},
  Author                   = {S. V. Zhidkov},
  Journal                  = {IEEE Trans. Consum. Electron.},
  Year                     = {2003},

  Month                    = {Nov. },
  Number                   = {4},
  Pages                    = { 944-948},
  Volume                   = {49}
}

@Article{Zhidkov2006,
  Title                    = {Performance analysis and optimization of {OFDM} receiver with blanking nonlinearity in impulsive noise environment},
  Author                   = {S. V. Zhidkov.},
  Journal                  = {IEEE Trans. Veh. Technol.},
  Year                     = {2006},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = { 234-242},
  Volume                   = {55}
}

@Article{zhou2014vector006,
  Title                    = {Vector orthogonal frequency division multiplexing system over fast fading channels},
  Author                   = {Zhou, Wen and Fan, Lisheng and Chen, Hongbin},
  Journal                  = {IET Commun.},
  Year                     = {2014},

  Month                    = {Sept.},
  Number                   = {13},
  Pages                    = {2322--2335},
  Volume                   = {8},

  Publisher                = {IET}
}

@Article{zhu2013simplified014,
  Title                    = {Simplified approach to optimized iterative clipping and filtering for {PAPR} reduction of {OFDM} signals},
  Author                   = {Zhu, Xiaodong and Pan, Wensheng and Li, Hong and Tang, Youxi},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {2013},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {1891--1901},
  Volume                   = {61}
}

@Article{Zimmermann02Apr,
  Title                    = {{A} multipath model for the powerline channel},
  Author                   = {Zimmermann, M. and Dostert, K.},
  Journal                  = {IEEE Trans. Commun.},
  Year                     = {Apr. 2002},
  Number                   = {4},
  Pages                    = {553-559},
  Volume                   = {50}
}


@INPROCEEDINGS{RabiePIMRC13, 
author={K. M. Rabie and E. Alsusa}, 
Booktitle  = {Proc. IEEE Pers. Indoor and Mobile Radio Commun. (PIMRC)},
title={Improving blanking/clipping based impulsive noise mitigation over powerline channels}, 
year={2013}, 
pages={3413-3417}, 
month={Sept.},
}

@INPROCEEDINGS{Bamidele06, 
author={B. Adebisi and B. Honary}, 
booktitle={Proc. IEEE Int. Symp. Power Lines Commun. and its Appl. (ISPLC)}, 
title={Comparisons of Indoor {PLC} Emissions Measurement Results and Regulation Standards}, 
year={2006}, 
pages={319-324}, 
month={Oct.},}

@article {Bamidele15,
author = {Gacanin, Haris and Adebisi, Bamidele and Ligata, Amir},
title = {Energy-efficient multiple-domain bidirectional scheme for {G}.hn applications},
journal = {Int. J. Commun. Syst.},
issn = {1099-1131},
year = {2015},
}

@INPROCEEDINGS{Bamidele11, 
author={A. Haidine and B. Adebisi and A. Treytl and H. Pille and B. Honary and A. Portnoy}, 
booktitle={Proc. IEEE Int. Symp. Power Lines Commun. and its Appl. (ISPLC)}, 
title={High-speed narrowband {PLC} in Smart Grid landscape - State-of-the-art}, 
year={2011}, 
pages={468-473}, 
month={Apr.},}

@INPROCEEDINGS{Bamidele14, 
author={B. Adebisi and A. Khalid and Y. Tsado and B. Honary}, 
booktitle={Proc. IEEE Int. Symp. Commun Syst., Net. Digital Signal Process. (CSNDSP)}, 
title={Narrowband {PLC} channel modelling for smart grid applications}, 
year={2014}, 
pages={67-72}, 
month={Jul.},}

@ARTICLE{Rabie15_SGT, 
author={K. M. Rabie and E. Alsusae}, 
journal={IEEE Trans. Smart Grid}, 
title={On Improving Communication Robustness in {PLC} Systems for More Reliable Smart Grid Applications}, 
year={2015}, 
volume={6}, 
number={6}, 
pages={2746-2756}, 
month={Nov.},}

@ARTICLE{Rabie15_AEU, 
author={K. M. Rabie and E. Alsusae}, 
journal={AEU-Int. J. Electron. Commun.}, 
title={Improved {DPTE} technique for impulsive noise mitigation over power-line communication channels}, 
year={2015}, 
volume={69}, 
pages={1847-1853}, 
month={Dec.},}

@ARTICLE{Zimmermann02Noise, 
author={M. Zimmermann and K. Dostert}, 
journal={IEEE Trans. Electromagn. Compat.}, 
title={Analysis and modeling of impulsive noise in broad-band powerline communications}, 
year={2002}, 
volume={44}, 
number={1}, 
pages={249-258}, 
month={Feb.},}

@ARTICLE{EMC_Gebhardt03, 
author={M. Gebhardt and F. Weinmann and K. Dostert}, 
journal={IEEE Commun. Mag.}, 
title={Physical and regulatory constraints for communication over the power supply grid}, 
year={2003}, 
volume={41}, 
number={5}, 
pages={84-90}, 
month={May},}

@INPROCEEDINGS{Adebisi_IET06, 
author={B. Adebisi and J. Stott and B. Honary}, 
booktitle={IET Int. Conf. Ionospheric Radio Systems and Techniques (IRST)}, 
title={Experimental study of the interference caused by {PLC} transmission on {HF} bands}, 
year={2006}, 
pages={326-330}, 
month={Jul.},}

@ARTICLE{Rabie16_SystemsJournal_EH, 
author={K. Maaiuf Rabie and B. Adebisi and A. M. Tonello and Galymzhan Nauryzbayev}, 
journal={IEEE Systems Journal}, 
title={For More Energy Efficient Dual-hop {DF} Cooperative Relaying PLC Systems}, 
year={2017}, 
volume={ }, 
note={},
number={ }, 
pages={1-12}, 
month={Jan.},}

@ARTICLE{VOFDM_Zhang05, 
author={Hong Zhang and Xiang-Gen Xia and L. J. Cimini and Pak Chung Ching}, 
journal={IEEE Trans. Wireless Commun.}, 
title={Synchronization techniques and guard-band-configuration scheme for single-antenna vector-{OFDM} systems}, 
year={2005}, 
volume={4}, 
number={5}, 
pages={2454-2464}, 
month={Sept.},}

@ARTICLE{Dubey15, 
author={A. Dubey and R. K. Mallik}, 
journal={IEEE Trans. Commun.}, 
title={{PLC} System Performance With {AF} {R}elaying}, 
year={2015}, 
volume={63}, 
number={6}, 
pages={2337-2345}, 
month={Jun.},}

@ARTICLE{Herath15, 
author={S. P. Herath, N. H. Tran and T. Le-Ngoc}, 
journal={IEEE Trans. Power Del.}, 
title={Optimal Signaling Scheme and Capacity Limit of {PLC} Under {B}ernoulli-{G}aussian Impulsive Noise}, 
year={2015}, 
volume={30}, 
number={1}, 
pages={97-105}, 
month={Feb.},}

@ARTICLE{Dubey15IET, 
author={A. Dubey and R. K. Mallik and R. Schober}, 
journal={IET Commun.}, 
title={Performance analysis of a multi-hop power line communication system over log-normal fading in presence of impulsive noise}, 
year={2015}, 
volume={9}, 
number={1}, 
pages={1-9}, 
month={Jan.},}



@ARTICLE{Ibo14_TSP, 
author={I. Ngebani and Y. Li and X. G. Xia and S. A. Haider and A. Huang and M. Zhao}, 
journal={IEEE Trans. Signal Process.}, 
title={Analysis and Compensation of Phase Noise in Vector {OFDM} Systems}, 
year={2014}, 
volume={62}, 
number={23}, 
pages={6143-6157}, 
month={Dec.},}


